Experimental Flight Testing of an Adaptive Autopilot with Parameter Drift Mitigation

This paper modifies an adaptive multicopter autopilot to mitigate instabilities caused by adaptive parameter drift and presents simulation and experimental results to validate the modified autopilot. The modified adaptive controller is obtained by including a static nonlinearity in the adaptive loop, updated by the retrospective cost adaptive control algorithm. It is shown in simulation and physical test experiments that the adaptive autopilot with proposed modifications can continually improve the fixed-gain autopilot as well as prevent the drift of the adaptive parameters, thus improving the robustness of the adaptive autopilot.

==> RCAC_section.tex <==

% \section{RCAC Algorithm}

This section briefly reviews the retrospective cost adaptive control (RCAC) algorithm. 
% In this work, retrospective cost adaptive control (RCAC) technique that is used to update the control law in a sampled-data feedback loop.
% RCAC is described in detail in \cite{rahmanCSM2017} and its extension to digital PID control is given in \cite{rezaPID}.
% The algorithm in \cite{rezaPID} is specialized for a PID control structure as shown in \cite{goel2020adaptive}.
% 
% Consider the control law
% \begin{align}
%     u_k 
%         =
%             \phi_k \theta_k,
%     \label{eq:uk_reg}
% \end{align}
% where, for all $k\ge0$, 
% the regressor $\phi_k \in \BBR^{l_u \times l_\theta}$ contains the measurements and $l_\theta$ depends on the structure of the controller.
% % 
% The controller coefficients $\theta_k \in \BBR^{l_\theta}$ are optimized by RCAC as described below. 
Consider a SISO PID controller with a feedforward term
\begin{align}
    u_k
        &=
            K_{\rmp,k} z_{k-1} +
            K_{\rmi,k} \gamma_{k-1} 
            \nn \\ &\quad +
            K_{\rmd,k} (z_{k-1} - z_{k-2}) +
            K_{{\rm ff},k} r_k
            ,
    \label{eq:uk_PID}
\end{align}
where $K_{\rmp,k}, K_{\rmi,k}, K_{\rmd,k}, $ and $K_{{\rm ff},k}$ are time-varying gains to be optimized, 
$z_k$ is an error variable,
$r_k$ is the feedforward signal, 
and, for all $k\ge0$,
%%\vspace{-5pt}
\begin{align}
    \gamma_k 
        \isdef
            \sum_{i=0}^{k} z_{i}.
\end{align}
%
%where $g \colon \BBR \to \BBR$ is an error normalization function.
%
Note that the integrator state is computed recursively using $\gamma_k = \gamma_{k-1} + g(z_{k-1})$.
% 
For all $k\ge0$, 
the control law can be written as 
\begin{align}
    u_k 
        =
            \phi_k \theta_k,
    \label{eq:uk_reg}
\end{align}
where 
the regressor $\phi_k$ 
and 
the controller gains $\theta_k$ 
% in \eqref{eq:uk_PID} 
are 
\begin{align}
    \phi_k
        \isdef
            \matl{c}
                z_{k-1} \\
                \gamma_{k-1} \\
                z_{k-1} - z_{k-2} \\
                r_k
            \matr^\rmT, \quad
    \theta_k
        \isdef
            \matl{c}
                K_{\rmp,k} \\
                K_{\rmi,k} \\
                K_{\rmd,k} \\
                K_{{\rm ff},k}
            \matr .
            % \in \BBR^{4}.
    \label{eq:phi_theta_def}
\end{align}
Note that the P, PI, or PID controllers can be represented by $\phi_k$ and $\theta_k$  by appropriately redefining these. For example,$\phi_k \isdef z_{k-1}$ and $\theta_k \isdef K_{\rmp,k}$ in the case of a P controller.
Various MIMO controller parameterizations are shown in \cite{goel_2020_sparse_para}.
% Note that $l_\theta=4$ in \eqref{eq:phi_theta_def}.

% \textbf{Add error normalization here}



% The controller structure for the proportional controller 

% The quadcopter is controlled by a digital controller operating in a sampled-data feedback loop.
%
% To describe the controller, we consider the SISO discrete-time plant
% \begin{align}
%     x_{k+1} 
%         &=
%             f(x_k,u_k,w_k), \\
%     y_k
%         &=
%             g(x_k,u_k,w_k), \\
%     z_k
%         &=
%             y_k - r_k,
% \end{align}
% where, for all $k\ge0$,
% $x_k \in \BBR^{l_x}$ is the state, 
% $u_k \in \BBR^{l_u}$ is the control signal,
% $w_k \in \BBR^{l_w}$ is the external disturbance, and
% $y_k \in \BBR^{l_y}$ is the measured output of the system,
% $r_k \in \BBR^{l_y}$ is the command signal, and
% $z_k \in \BBR^{l_y}$ is the performance variable. 
%
%
% In particular, consider the  PID controller  
% %%\vspace{-5pt}
% \begin{align}
%     u_k
%         =
%             K_{\rmp,k} z_{k-1} +
%             K_{\rmi,k} \gamma_{k-1} +
%             K_{\rmd,k} (z_{k-1} - z_{k-2}),
%     \label{eq:uk_PID}
% \end{align}
% where $K_{\rmp,k}, K_{\rmi,k}, K_{\rmd,k}$ are time-varying gains to be adapted, $z_k$ is an error variable, and, for all $k\ge0$,
% %%\vspace{-5pt}
% \begin{align}
%     \gamma_k 
%         \isdef
%             \sum_{i=0}^{k} z_{i}.
% \end{align}
% Note that the integrator state can be computed recursively using $\gamma_k = \gamma_{k-1} + z_{k}$.
% %
% Finally, note that the control \eqref{eq:uk_PID} can be written as
% %%\vspace{-10pt}
% \begin{align}
%     u_k 
%         =
%             \phi_k \theta_k,
%     \label{eq:uk_reg}
% \end{align}
% where, for all $k\ge0$,
% %%\vspace{-10pt}
% \begin{align}
%     \mspace{-8mu}\phi_k
%         \isdef
%             [
%                 z_{k-1} \ \
%                 \gamma_{k-1} \ \
%                 z_{k-1} - z_{k-2}
%             ], \quad
%     \theta_k
%         \isdef
%             \matl{c}
%                 K_{\rmp,k} \\
%                 K_{\rmi,k} \\
%                 K_{\rmd,k}
%             \matr.
%     \label{eq:phi_theta_def}
% \end{align}

To determine the controller gains $\theta_k$, let $\theta \in \BBR^{l_\theta}$, and consider the \textit{retrospective performance variable} defined by
%%\vspace{-5pt}
\begin{align}
    \hat{z}_{k}(\theta)
        \isdef
            z_k + 
            \sigma (\phi_{k-1} \theta - u_{k-1}),
    \label{eq:zhat_def}
\end{align}
where $\sigma \in \BBR.$
The sign of $\sigma$ is the sign of the leading numerator coefficient of the transfer function from $u_k$ to $z_k.$
%
Furthermore, define the \textit{retrospective cost function} $J_k \colon \BBR^{l_\theta} \to [0,\infty)$ by
%%\vspace{-10pt}
\begin{align}
    J_k(\theta) 
        &\isdef
            \sum_{i=0}^k
                \hat{z}_{i}(\theta) ^\rmT 
                R_z
                \hat{z}_{i}(\theta)
                 +
                (\phi_k \theta)^\rmT
                R_u
                (\phi_k \theta)
                \nn \\ &\quad \quad +
                (\theta-\theta_0)^\rmT 
                P_0^{-1}
                (\theta-\theta_0),
    \label{eq:RetCost_def}
\end{align}
where $R_z, R_u \in \BBR,$ $\theta_0\in\BBR^{l_\theta}$ is the initial vector of PID gains and $P_0\in\BBR^{l_\theta\times l_\theta}$ is positive definite.
%
% For all examples in this paper, we set $\theta_0 = 0$; however, $\theta_0$ can be initialized to nonzero gains in practice if desired.



\begin{proposition}
    Consider \eqref{eq:uk_reg}--\eqref{eq:RetCost_def}, 
    where $\theta_0 \in \BBR^{l_\theta}$ and $P_0 \in \BBR^{l_\theta \times l_\theta}$ is positive definite. 
    Furthermore, for all $k\ge0$, denote the minimizer of $J_k$ given by \eqref{eq:RetCost_def} by
    \begin{align}
        \theta_{k+1}
            \isdef
                \underset{ \theta \in \BBR^n  }{\operatorname{argmin}} \
                J_k({\theta}).
        \label{eq:theta_minimizer_def}
    \end{align}
    Then, for all $k\ge0$, $\theta_{k+1}$ is given by 
    \begin{align}
        \theta_{k+1} 
            &=
                \theta_k  - 
                 \sigma P_{k+1}\phi_{k-1}^\rmT R_z
                 [ z_k + \sigma(\phi_{k-1} \theta_k - u_{k-1}) ]
                 \\ &\quad \quad 
                 - 
                 P_{k+1}\phi_{k}^\rmT
                 R_u \phi_{k} \theta_k 
                 , \label{eq:theta_update}
    \end{align}
    where 
    \begin{align}
        P_{k+1} 
            &=
                P_{k}
                -  
                P_k  
            \Phi_k ^\rmT 
            \left( 
                \bar R ^{-1} +  
                \Phi_k
                P_k
                \Phi_k ^\rmT 
            \right)^{-1}
            \Phi_k,
        \label{eq:P_update_noInverse}
    \end{align}
    and
    \begin{align}
        \Phi_k
            \isdef 
            \matl{c}
                \sigma \phi_{k-1} \\
                \phi_k
            \matr,
        \quad 
        \bar R
            \isdef 
                \matl{cc}
                    R_z & 0 \\
                    0   & R_u
                \matr.
    \end{align}
    % \begin{align}
    %     P_{k+1} 
    %         &=
    %             P_{k}
    %             -  \frac
    %                 { P_{k}\phi_{k-1}^\rmT  \phi_{k-1} P_{k} }
    %                 { 1 +   \phi_{k-1} P_{k} \phi_{k-1}^\rmT  }.
    %     \label{eq:P_update_noInverse}
    % \end{align}
\end{proposition}
\begin{proof}
See \cite{AseemRLS}.
\end{proof}

Finally, the control is given by
\begin{align}
    u_{k+1} = \phi_{k+1} \theta_{k+1}.
\end{align}
